Self-Supervised Polyp Re-Identification in Colonoscopy

Computer-aided polyp detection (CADe) is becoming a standard, integral part of any modern colonoscopy system. A typical colonoscopy CADe detects a polyp in a single frame and does not track it through the video sequence. Yet, many downstream tasks including polyp characterization (CADx), quality metrics, automatic reporting, require aggregating polyp data from multiple frames. In this work we propose a robust long term polyp tracking method based on re-identification by visual appearance. Our solution uses an attention-based self-supervised ML model, specifically designed to leverage the temporal nature of video input. We quantitatively evaluate method's performance and demonstrate its value for the CADx task.

==> sections/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> sections/optical_biopsy_backup.tex <==
Optical biopsy, namely, using artificial intelligence for computer-aided diagnosis (CADx), has the potential to decrease the costs and workloads of polypectomy and pathology for the health system. Endoscopic characterization of colorectal polyps to be either neoplastic or non-neoplastic (e.g. hyperplastic) in real time can allow the implementation of \textit{resect-and-discard} and \textit{leave-in-situ} strategies, where selected polyps can be discarded without undergoing the pathology inspection process, or left unresected, as they don't present any risk of developing into Colorectal Cancer (CRC). Using a real-time system to accurately characterize the type of detected polyps is crucial for the implementation of such strategies.

The development of robust and accurate methods for optical diagnosis remains a challenge for researchers and the healthcare community, despite several publications demonstrating promising results (see for example, \cite{hassan2022artificial,zachariah2020prediction,biffi2022novel}). Some studies have concluded that current systems do not improve results when compared to procedures conducted without the assistance of CADx \cite{barua2022real}. Moreover, recently the World Endoscopy Organization (WEO) provided its perspective regarding the use of CADx \cite{mori2023benefits}, and recommended continuing research in this area, pointing out that CADx must be sufficiently accurate in order to reduce healthcare costs. By developing more accurate and robust systems, CADx can become a standard practice in real-world colonoscopy.

The majority of CADx systems provide a classification score for each frame, followed by an aggregation of scores to determine a final prediction of the polyp diagnosis. A common aggregation mechanism is a simple voting procedure \cite{biffi2022novel}. Other aggregation methods include average score and temporal smoothing \cite{byrne2019real}. In all of the above, longer sequences, with a large number of frames, should provide more information necessary to get an accurate prediction. The association of a sequence of frames into a single polyp tracklet is a critical part of the algorithm, usually based on spatial tracking, or by manually annotating selected frames \cite{byrne2019real,mori2018real,nogueira2021deep}. Several reported methods mention as a requirement that the observed polyp should be framed consistently \cite{biffi2022novel}. Such requirements are often strict and require the physician to alter the normal execution of tasks in real-life colonoscopy \cite{hassan2022artificial}. Furthermore, an ideal system would benefit from viewing the polyp from multiple angles. Such navigation around the polyp is difficult even for expert physicians, and can easily cause the polyp to get out of the endoscope field of view. Grouping multiple consistent sequences into a single tracklet can potentially enhance the the accuracy in such scenarios. Here, we show that using the suggested ReID model to group separate tracklets can increase the performance of CADx system, with no minimum requirements regarding the video quality.

\subsection{Data}
To train and evaluate a deep convolutional neural network (CNN) to predict the characterization of a polyp frame, we used a second private dataset, taken from $3290$ colonoscopy procedures videos that were not used at any stage to train or evaluate the ReID model. The videos were recorded as part of standard colonoscopy procedures, without the use of CAD systems. First, we used the pre-trained tracking-by-detection model to find the frames containing polyps from within each procedure. An expert physician annotated key frames of each polyp, allowing the association of multiple tracklets to a single sequence, even after encountering occlusions and loss of tracking. Then, each polyp was annotated to be either adenoma or non-adenoma by an expert physician. We randomly sampled the procedures to train, validation, and test set ($2666$, $296$, and $328$ procedures respectively). Unfortunately, golden standard histology reports were not available for this dataset.


\subsection{Experiments}
We trained a simple classification CNN, consisting of a MobileNet \cite{sandler2018mobilenetv2} backbone, followed by an MLP layer with a Sigmoid activation, to predict a score in range 0 (non-adenoma) and 1 (adenoma) for each frame. The model was trained for 200 epochs with a learning rate of $0.001$ and Adam optimizer \cite{kingma2014adam}. The best checkpoint was chosen using evaluation over the validation set.

\subsubsection{Effect of the Sequence Length on CADx Performance}
\todo{add this section if there is room left.}

\subsubsection{ReID Based CADx Performance}
To assess the benefit of using Re-ID as part of the optical diagnosis, we compared the results of the CADx system on the test set, while using different grouping methods to associate multiple frames into polyp tracklets. We compared the performance on 3 variations of the test set - the original annotated data, tracking-based data, and ReID-based data. As the golden baseline, we used the annotated polyp sequences. Those are the longest sequences, containing all of the frames of each polyp in the test set. To simulate the results of using a spatial tracking mechanism as the grouping method, we separated each annotated tracklet into several tracklets, by generating a new tracklet each time the detector lost track for more than 15 consecutive frames. Then, we used the ReID model to merge the generated tracklets, to get the ReID-based data. The characterization label of the generated tracklets remains the same as that of the original annotated tracklet. A visualization of the separation and grouping process is described in figure \ref{fig:data_split}. Following this scheme, the annotated test set has a fragmentation rate of $1.0$ by definition, while the tracking-based test set and ReID-based test set have fragmentation rates of $5.20$ and $1.68$ respectively. \todo{add a note of how this connects to the ReID benchmark above.} All 3 dataset variations are composed of the same procedures and frames, and the only difference between them is the grouping into tracklets. The number of tracklets in each dataset and the class label distribution appear in table \ref{table:ob_data_dist}.

\begin{figure}
\includegraphics[width=1\textwidth]{figures/ob_data_split.png}
\caption{Separation of the annotated polyp into tracking and ReID-based tracklets. All rows display the same sequence of frames, while each color represents a single tracklet. Frames where no polyp was detected, appear uncolored. 3 tracklets are generated from the ground truth tracklet, then merged back into 2 distinct tracklets by the ReID model.}
\label{fig:data_split}
\end{figure}

\begin{table}
\centering
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
\begin{tabular}{ |p{1.65cm}|p{1.4cm}|p{1cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{2.2cm}| } 
\hline
Grouping Method & Tracklets & FR & Adenoma & Adenoma FR & Non-Adenoma & Non-Adenoma FR \\
\hline
Annotation & $608$ & $1.0$ & $464$ & $1.0$ & $144$ & $1.0$ \\
Tracking & $3161$ & $5.20$ & $2537$ & $5.47$ & $624$ & $4.33$\\
ReID & $1023$ & $1.68$ & $813$ & $1.75$ & $210$ & $1.46$\\
\hline
\end{tabular}
\caption{Optical Biopsy test set data distribution and fragmentation rate (FR) for each grouping method. The annotated dataset consists of 608 polyps with a single annotated tracklet for each of them, hence has a FR of $1.0$. }
\label{table:ob_data_dist}
\end{table}

We used the same classification model to evaluate all 3 grouping methods. We used the model to predict the classification score for each frame and aggregated the scores of each tracklet to achieve the final prediction score. The aggregation was performed using voting. We compare the $F_1$ measure, as well as the $AUC$. In addition, we measured the sensitivity for each method, while setting a specificity threshold of $0.9$. The results are summarized in table \ref{table:ob_resuls}. As expected, grouping by tracking leads to a drastic degradation in performance in comparison to annotation-based grouping. When employing the ReID model, the performance significantly improves. 

\begin{table}
\centering
\begin{tabular}{ |c|c|c|c|c| } 
\hline
Grouping Method & AUC & F1 (Macro) & F1 (Micro) & Sensitiviy @ Specificity=0.9 \\
\hline
Annotation &  0.95 & 0.88 & 0.91 & 0.86 \\
ReID & 0.90 & 0.82 & 0.88 & 0.79 \\
Tracking & 0.86  & 0.77 & 0.83 & 0.71 \\
\hline
\end{tabular}
\caption{Optical Biopsy Result Per Grouping Method.}
\label{table:ob_resuls}
\end{table}

